Morshed: Guiding Behavioral Decision-Makers towards Better Security Investment in Interdependent Systems

We model the behavioral biases of human decision-making in securing interdependent systems and show that such behavioral decision-making leads to a suboptimal pattern of resource allocation compared to non-behavioral (rational) decision-making. We provide empirical evidence for the existence of such behavioral bias model through a controlled subject study with 145 participants. We then propose three learning techniques for enhancing decision-making in multi-round setups. We illustrate the benefits of our decision-making model through multiple interdependent real-world systems and quantify the level of gain compared to the case in which the defenders are behavioral. We also show the benefit of our learning techniques against different attack models. We identify the effects of different system parameters on the degree of suboptimality of security outcomes due to behavioral decision-making.

==> Incomplete_Information_Setup.tex <==
\section{Incomplete Information Sharing among defenders}\label{sec:incomplete-information-games}
\vspace{-0.1cm}

So far we have considered in our formulation that each defender has complete information about the other defenders (their behavioral level, total budget, etc.). However, in many practical security scenarios, a defender may only have incomplete information about the others (e.g., the defenders may refrain from revealing (all) their information to others defending the interdependent system) akin to the notion of ``Incomplete-Information" that has been used in behavioral economics literature (e.g., \cite{harsanyi1967games}). Multiple studies \cite{stahl1994experimental,nagel1995unraveling} showed by subject experiments that complete-information model is not the only model to study the humans' interactions. In this context, the seminal paper \cite{nagel1995unraveling} showed that subjects in their experiments have never made equilibrium guesses. This motivates the model of ``Incomplete-information" that we consider here in the context of security of interdependent systems.

% In Section~\ref{sec:securitygames}, we considered outcomes in which each defender mutually best responds to other defenders' investments when having a complete information model of the other defenders.  Thus, we use the notion of ``Incomplete-Information" which was used in behavioral economics literature (e.g., \cite{stahl1994experimental,costa2006cognition}) that  %\footnote{TC(9/30/19) These level-k references are not the right ones. The uncertainty described in the next paragraph is for a Bayesian game of incomplete information, and the Bayesian Nash equilibrium is the right solution concept. Harsanyi (1967/1968) is the seminal reference. Is this the solution concept you are using?}
% \footnote{\color{blue}{PN(10/1/19): I would like to second Tim's earlier comment here. It is not clear if we are using BNE (which seems to be the right way of thinking about incomplete information) or k-level reasoning (which to my understanding is a model of bounded rationality)?}}
% \textbf{The incomplete information game:}
In a game of incomplete information, each defender has partial knowledge about other defenders in the system. Here, we consider the following two forms of incomplete information: each defender does not know the others' defense budgets, and each defender does not know the behavioral level ($\alpha$) of the other defenders referred to as {\bf $B$-Incomplete-information} and {\bf $\alpha$-Incomplete-information}, respectively.
We analyze how the security under such partial knowledge compares to that under complete information. 

In modeling partial knowledge, defenders assume a probability distribution over the unknown parameter. That is, 
a defender $D_k$ assumes that other defenders' (unknown) %can have different discrete levels of security budget or different discrete levels of behavioral level, 
security budgets or behavior levels are distributed according to some probability distribution $P_0$ over admissible (discrete) budgets or behavioral levels, respectively. 
To select her investments, defender $D_k$ computes her best response to the expected profile of strategies of other defenders given $P_0$; this is the expected value of investment vectors where each vector corresponds to one discrete budget/behavior level. 

In our evaluation, we will show that the benefit of greater information sharing  diminishes as the defenders become more rational (or less behavioral) and show the importance of such sharing in interdependent systems.

%is confusing as written and we do not have space to explain in detail. 
% Note that such investment vector for each defender $D_j, j\neq k$ is the optimal investment decision of that defender, i.e., $D_j$, where $D_j$ assumes that defender $D_k$ has no investments. This model is named level-k reasoning \cite{costa2006cognition,stahl1994experimental} where in our setup, each defender $D_k$ is considered to be level-2.
% Below, we compare the ratio of total system loss incurred by defenders in incomplete-information to complete-Information, for both $B$-Incomplete-Information $\alpha$-Incomplete-Information games. 
%Here, we compare the total system loss due to defense placement by non-behavioral defender and the total system loss due to defense placement by behavioral defender for different behavioral levels in all of the three security games variants: $B$-Incomplete-Information, $\alpha$-Incomplete-Information, and Complete-Information (PNE). We repeat the experiment for all three budget levels that we defined earlier where we consider symmetric budget distribution between the defenders to isolate other factors.

\begin{comment}
\begin{figure}[htbp]
\begin{minipage}[t]{0.48\linewidth}
    \includegraphics[width=\linewidth,keepaspectratio]{Figures/DER_Incomplete_alpha_all.pdf}
  \caption{The total loss for different budgets and different behavioral levels for $B$-incomplete-information game for DER.1.}
  \label{fig:Incomplete_BR_DER}
\end{minipage}%
    \hfill%
\begin{minipage}[t]{0.48\linewidth}
        \includegraphics[width=\linewidth,keepaspectratio]{Figures/Scada_BR_Incomplete.pdf}
  \caption{The total loss for different budgets and different behavioral levels for $B$-incomplete-information game for SCADA.}
  \label{fig:Incomplete_BR_SCADA}
\end{minipage} 
%\vspace{-0.080in}
\end{figure}
\end{comment}




==> Makefile <==
#
# Makefile for acmart package
#
# This file is in public domain
#
# $Id: Makefile,v 1.10 2016/04/14 21:55:57 boris Exp $
#

PACKAGE=acmart

SAMPLES = \
	ccs-template.tex 

PDF = $(PACKAGE).pdf ${SAMPLES:%.tex=%.pdf}

all:  ${PDF}

%.pdf:  %.dtx   $(PACKAGE).cls
	pdflatex $<
	- bibtex $*
	pdflatex $<
	- makeindex -s gind.ist -o $*.ind $*.idx
	- makeindex -s gglo.ist -o $*.gls $*.glo
	pdflatex $<
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $*.log) \
	do pdflatex $<; done


acmguide.pdf: $(PACKAGE).dtx $(PACKAGE).cls
	pdflatex -jobname acmguide $(PACKAGE).dtx
	- bibtex acmguide
	pdflatex -jobname acmguide $(PACKAGE).dtx
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' acmguide.log) \
	do 	pdflatex -jobname acmguide $(PACKAGE).dtx; done

%.cls:   %.ins %.dtx  
	pdflatex $<

%.pdf:  %.tex   $(PACKAGE).cls ACM-Reference-Format.bst
	pdflatex $<
	- bibtex $*
	pdflatex $<
	pdflatex $<
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $*.log) \
	do pdflatex $<; done

sample-manuscript.pdf \
sample-acmsmall.pdf \
sample-acmlarge.pdf \
sample-acmtog.pdf: samplebody-journals.tex

sample-sigconf.pdf \
sample-sigconf-authordraft.pdf \
sample-sigplan.pdf \
sample-sigchi.pdf: samplebody-conf.tex


.PRECIOUS:  $(PACKAGE).cfg $(PACKAGE).cls


clean:
	$(RM)  $(PACKAGE).cls *.log *.aux \
	*.cfg *.glo *.idx *.toc \
	*.ilg *.ind *.out *.lof \
	*.lot *.bbl *.blg *.gls *.cut *.hd \
	*.dvi *.ps *.thm *.tgz *.zip *.rpi

distclean: clean
	$(RM) $(PDF) *-converted-to.pdf

#
# Archive for the distribution. Includes typeset documentation
#
archive:  all clean
	tar -C .. -czvf ../$(PACKAGE).tgz --exclude '*~' --exclude '*.tgz' --exclude '*.zip'  --exclude CVS --exclude '.git*' $(PACKAGE); mv ../$(PACKAGE).tgz .

zip:  all clean
	zip -r  $(PACKAGE).zip * -x '*~' -x '*.tgz' -x '*.zip' -x CVS -x 'CVS/*'


==> Min_Cut_results.tex <==
\section{Guiding Security Decision-Makers in one round} \label{sec:guiding_min_cut}
Our example in Section~\ref{sec:theory}, and its intuitive interpretations, illustrate how behavioral biases in security decision making (the existence of which is also supported by our human subject study described in Section~\ref{sec:human-experiments}) negatively affect interdependent systems' security. Motivated by these findings, we next propose algorithms to guide a behavioral security decision-maker (here, the human defender of the interdependent system) to invest only on critical edges. In this section, we propose such method when the algorithm interacts with the decision-maker only once. 

\subsection{Proposed Algorithm}
The following pseudo-code describes the steps used for guiding the decision-maker to distribute her security resources optimally for a given attack graph. Note that the simpler version of such problem has been studied in the literature for considering only one single target using different methods (e.g., using graph-theoretic cuts \cite{dickerson2010graph}).\pn{8/11}{This sentence unclear. We do not develop min-cut, and min-cut is just an example of a graph-theoretic cut.} However, no automated way was proposed to optimize allocations for multiple targets (by forcing to invest only on min-cut edges). \pn{8/11}{Overall, the claims on this algorithm and its contributions should be dialed down in my opinion. This seems like an iterated application of min-cut.}

Our proposed algorithm,  Algorithm 1, invokes the \texttt{min\_cut} algorithm multiple times, each time with one of the critical assets as its sink node. 
%We begin by checking that the array of indices of critical assets is not empty. Second, we iterate over each critical asset and 
Each such call to \texttt{min\_cut} outputs the minimum edge cut between this critical asset and the source asset (the entry point $v_s$). We append the set of edges in this edge cut to a set $\mathcal{O}$, then remove them from the graph. The graph containing the set of remaining edges is passed on to the next iteration of the algorithm. The algorithm continues until no more critical assets remain.  
%Then, we remove the edges between the current critical asset and previous critical assets to avoid getting repeated edges in the resultant edge set. 
After finishing the process, the resultant set of edges $\mathcal{O}$ is given to the behavioral defender, who then minimizes the total loss function in \eqref{eq:defender_utility_edge} under the constraint of only investing on the edges in $O$. 
%(extracted by first part of our algorithm).
% \cite{west2001introduction} 

\pn{8/11}{Again, I am not a fan of this algorithm and the section overall. If we are giving the decision maker a set of edges to invest on, why not just straight out tell them how much to invest on each? Also, what difference does it make to allow the behavioral defender to run the optimization problem once we give them the edge cut? If there is something I'm missing, please clarify.}
\pn{8/12}{You are correct. I will drop this whole small section.}

\iffalse
\noindent \textbf{Complexity of the algorithm:} Note that multiple algorithms were proposed for finding (minimal or minimum) edge cuts between $v_s$ and $v_m$. The Edmonds-Karp algorithm \cite{cormen2001introduction} selects minimal sets (w.r.t. set inclusion) of vertices reachable from $v_s$ in the final residual graph with a running time of $O(|V| \cdot|E|^{2})$. Moreover, the enhanced method of this algorithm known as Dinic's algorithm \cite{dinic1970algorithm} has better performance ($O(|V|^{2} \cdot|E|)$ or better).
\fi

\SetKwInput{KwInput}{Input}
\SetKwInput{KwOutput}{Output}
\begin{algorithm}%[t]
  \KwInput{DAG $G = (\mathcal{V} , \mathcal{E})$ and ordered set of critical assets, $V_m$}
  \KwOutput{Set of edges to place investments on, $\mathcal{O}$}
 % current\_critical\_asset\_index = $v_i$ =  0
  
  \For{ $v_m  \in  V_m$}
    {
        \For{each predecessor critical asset $v_n$ of $v_m$}
        {
            
            \If{$ (v_n,v_m) \in \mathcal{E}$}
            {
              Remove Edge $(v_n,v_m)$ from $\mathcal{E}$     
            }
        }

        \textbf{Call} min\_cut  ($v_s$,$v_m$) 
        
        %\pn{is min-edge-cut the same thing as min-cut? Choose to use one name consistently.}
        %\mustafa{8/12}: Done
        
        Append result of min\_edge\_cut ($v_s$,$v_m$) to $\mathcal{O}$ 
    }
    Minimize total loss function in \eqref{eq:defender_utility_edge}
    s.t. $x_{i,j} > 0$ if $(v_i,v_j) \in \mathcal{O}$
    %    remove selected rule from remaining rule list
%    }
\caption{Determining critical defense edges in a network with multiple critical assets}
\end{algorithm}

%Second, we assume that the best value of k lies in a range from A to B (initially set to either the tool’s recommended range, or between 1 and L, where L is the read size). We apply an existing EC algorithm (Lighter, Blue, or RACER in our evaluation) with different initial values (k0, ···, km)∈(A,B), to avoid getting stuck in local minima, going through multiple iterations for a given initial value.


Note that this kind of defense of min-ct edges is represented in real scenarios. For instance, Real defenders use similar defenses when they install a firewall at the boundary between their organization and the Internet.

\iffals
\pn{8/11}{My verdict based on reading so far is that this whole section be dropped. Is there a particular reason this has been added in the first place? I don't know if this complements any of the results in the remainder of the paper though.}

\mustafa{8/12}{I agree with you. I was also discussing with Saurabh about its limitations and that Cost function of Rational defender can be solution for one round.}
\fi

==> README <==
This package provides a class for typesetting publications of 
Association for Computing Machinery.

Your TeX distribution probably includes the latest released version of
this package.  If you decide to install it yourself, please see
Installation section of the User's Guide.

Changes

version 1.08    SIGPLAN reformatting (Matthew Fluet); bug fixes

version 1.09    SIGPLAN: revert caption rules (Matthew Fluet)

version 1.10    Bug fixes

version 1.11    Customization of ACM theorem styles and proof
                environment (Matthew Fluet).

version 1.12    Bug fixes and documentation updates.  
		Footnotes rearranged.
                Option natbib is now mostly superfluous: the class 
		makes a guess based on the format chosen.

version 1.13    Formatting changes: headers, folios etc.
		Bibliography changes.

version 1.14    Warn about undefined citation styles; move definitions
                of acmauthoryear and acmnumeric citation styles before
                use.

version 1.15    New structured affiliation command.
                New commands for acknowledgements.

version 1.16    Formatting changes for headers and footers.

version 1.17    Formatting changes for margins and lists.  Bug fixes.

version 1.18    Natbib is now the default for all versions.  A unified bib
		file is used for all styles.  Better treatment
		of multiple affiliations.

version 1.19    Include 'Abstract', 'Acknowledgements', and 'References'
                in PDF bookmarks.

version 1.20    Bug fixes, documentation updates

version 1.21    Bibliography changes: added arXiv, some cleanup

version 1.22    Bibliography changes for Aptara backend;  should be 
		invisible for the users.

version 1.23    Added PACM PL journal option.

version 1.24    Added IMWUT journal option.

version 1.25    Updated PACMPL journal option.

version 1.26    Bug fixes

version 1.27    Bug fixes

version 1.28    Bug fixes: natbib=false now behaves correctly.

version 1.29	Documentation changes.  Head height increased from 12pt to 13pt.
		Removed spurious indent at start of abstract.
		Improved kerning in CCS description list.

version 1.30    Bibtex style now recognizes https:// in doi.
	        Added \frenchspacing.
		\department now has an optional hierarchy level.
		Switched to T1 encoding
		Updated IMWUT and PACMPL

version 1.31    Changed default year and month to the current ones
		(thanks to Matteo Riondato)
		Table of contents now works
		Marginalia now work in all formats
		New command \additionalaffiliation
		Documentation changes

version 1.32    New DOI formatting.
		Format siggraph is now obsolete, and sigconf
		is used instead.
		New proceedings title: POMACS.

version 1.33    New option `timestamp' (Michael D. Adams)
		New option `authordraft'
                Documentation updates
		Bug fixes
		We now use Type 1 versions of Libertine fonts even with XeTeX.
		New hook acmart-preload-hook.tex (wizards only!)
		Added new options `obeypunctuation' for \affiliation command
		Added SubmissionID
		Added right line count ruler for two-column formats
		Added workaround for Adobe Acrobat bugs in selection
		Added eid field to the bibliography
		
version 1.34    Deleted DOI from doi numbers
		Changed bibstrip formatting
		The command \terms is now obsolete
		The rulers in review mode now have continuous numbering

version 1.35    Author-year bib style now uses square brackets.
		Changed defaults for TOG sample
		Price is suppressed for usgov and rightsretained modes.
		Bugs fixed

==> Scada_Case_Study.tex <==
\section{CPS Study: SCADA Control System}\label{sec:scada}

\begin{figure}[t]
\begin{center}
  \includegraphics[width=0.9\linewidth,height=60mm,keepaspectratio]{Figures/Scada_nonum_attack_graph.pdf}%Attack_Graph_Scada.pdf
  \caption{The attack graph for a SCADA-based control network, adapted from \cite{hota2016optimal}. The attacker's starting node is $S$. Each target node has an associated loss (denoted as L within the node).}%The initial attack success probabilities are shown on the edges.
  \label{fig:Scada_attack_Graph}
  \end{center}
  \vspace{-0.2in} 
\end{figure}
%PN(10/28/18): The graph looks great! Thanks for revising Mustafa. 

\begin{figure*}[t] 
%\centering
\begin{minipage}[t]{1.0\textwidth}
\begin{minipage}[t]{.32\textwidth}
\centering
\includegraphics[width=\linewidth]{Figures/Scada_BT_Behavioral_Effect.pdf}
\caption{Total loss of the SCADA-based system as a function of budget. The effects of human behavior decision making are high for this attack graph, due to the increase in the degree of interdependency and the number of critical assets.}% $ BT $ is the total available security budget for all defenders.}
\label{fig:Effect_BT_Behavioral_Scada}
\end{minipage}\hfill
\begin{minipage}[t]{.32\textwidth}
\centering
\includegraphics[width=\linewidth]{Figures/Scada_NumRTUs_Effect.pdf}
\caption{Total loss as a function of the number of RTUs per defender. %where $ BT = \$25$. 
We observe that the effect of increasing the number of critical assets is more pronounced when the degree of behavioral decision making is higher %(i.e., $\alpha$ decreases ) 
as the suboptimal decisions affects all critical assets.% (RTUs) of the player's subnetwork.
}
\label{fig:Scada_Effect_RTUs}
\end{minipage}\hfill
\begin{minipage}[t]{.32\textwidth}
\centering
  \includegraphics[width=\linewidth]{Figures/Joint_indiv_comparison.pdf}
  \caption{ Comparison between individual defense and joint defense investment mechanisms. We observe that joint defense can outperform individual defense (i.e., lower losses), particularly when behavioral probability weighting is higher (i.e., lower $\alpha$). %We fix the security budget ( $ BT $ ) distribution at $\frac{1}{3}$ and $\frac{2}{3}$ for defenders 1 and 2 respectively.
  } 
\label{fig:Effect_Joint_Behavioral_Scada}
\end{minipage}
%  \label{figure:Synthetic_Errors_Detection}
\end{minipage}
%\vspace{-0.1in}
\end{figure*}


\subsection{Results and insights}
% SB (5/14/19): Chopped for space
\begin{comment}
In this section, we introduce one new experiment to identify if there is a benefit to centralized planning of security controls (Experiment B.5). Other experiments verify the intuitions of DER but the difference between the behavioral and the non-behavioral losses is magnified due to the greater degree of interdependency and the larger number of critical assets. Also, the scaling experiment brings out a more rapid increase in loss for behavioral players than in the DER system. 
\end{comment}

%\subsubsection*
\vspace{0.01in}



%\subsubsection*
\vspace{0.01in}
\noindent {\em\textbf{Experiment 2: Number of critical assets. }} Here we consider scaling up the SCADA system, with each defender owning more physical assets and correspondingly having a larger number of RTUs. We make replicas of these RTUs for each defender, and assume that the defender has the same security budget $BT=25$, done to measure the effect of suboptimal decisions as the CPS size grows. Again, we notice that as the number of RTUs increases, the difference between system loss with behavioral players versus non-behavioral players is magnified as shown in Figure \ref{fig:Scada_Effect_RTUs}. For instance, we observe that when $ \alpha= 1 $, a change from 3 RTUs per player to 18 RTUs per player yields a relative increase of $ 344\% $ in system loss, while the same change with $ \alpha = 0.4 $ results in a higher increase of $ 882\%$. As the size of the CPS grows, the budget stays constant and hence the magnitude of the loss increases.
As the decision becomes behavioral, at large CPS sizes, the scarce defense budget is improperly allocated and this magnifies the loss. 
The impact of behavioral decisions is more damaging here than in the DER case because of the highly critical edges between the control network and the RTUs. A non-behavioral defender protects these critical edges, but a behavioral one mistakenly distributes her budget between these and other edges.

% \issa{I wonder what will happen if you increase the number of RTUs more 100, 200, 1000, ... while keeping fixed budget. The intuition is that both behavioral and non behavioral defenders will meet at some point. I think it is good to show something like this.}
% \mustafa{I think as Figure 17 shows, as number of RTUs increases, the difference will be higher between behavioral and non-behavioral. The reason is that each added new RTU will be associated with non-common edge from control unit to RTU where behavioral defender puts non-zero investments.}


\vspace{0.01in}
\noindent {\em\textbf{Experiment 4: Centralized defense merits.}}
Next, we compare the outcomes of decentralized decision-making by two defenders with a centralized defense method where a central planner owns both subnetworks and aims to minimize the system loss % (i.e., the sum of expected losses of all critical units) of all defenders) 
by allocating the budget appropriately. %minimization in which a central planner (e.g., official authority) takes care of minimizing th 
%We note that in centralized defense the game is just a single player (i.e., official authority ) that takes the responsibility of distributing the budget on the whole huge network. 
We observe that when the defenders have a symmetric budget, the outcomes of central and distributed planning coincide. As the budget asymmetry increases, the difference between the two defense methods increases as well. Figure \ref{fig:Central_Behavioral_Scada} shows this trend for two budget choices, $ BT = 10$ and $ BT = 20$. We observe that with the lower budget, the suboptimality due to selfish decision making is more pronounced. 
Further, we observe that interventions by a social planner have a higher benefit %of the system 
when the defenders are behavioral. % decision makers. 
In particular, when $ BT = 10 $, the relative difference between social and selfish for $ \alpha = 1 $ is $5.7\%$, while it is higher (14\%) for $ \alpha=0.6 $.
% SB (10/31/18): Be more quantitative to make a point - is the difference 1% (in which case we do not have a strong point) or is it 50%?
% Mus(10/31/18): 14% at alpha = 0.6, 5.7% at alpha = 1. Added. Thinking of removing "Further,..". 
% SB (11/1/18): Resolved.

A well-known metric, called the Price of Anarchy (PoA) is often used to quantify the inefficiency of Nash equilibrium~\cite{roughgarden2005price}. PoA equals the ratio of the highest total system loss at any PNE and the total system loss at the social optimum. 
% In this experiment, for fair comparison, we use optimistic PoA which equals the ratio of the total loss at the best PNE (with equal budget distribution among players) and that at the social optimum. 
Figure \ref{fig:POA_Behavioral_Scada} illustrates the (optimistic) PoA for different available security budgets. We observe that the PoA increases as the players become more behavioral, particularly for higher available security budgets. An interesting observation here is that although at higher budgets total system loss is close to zero and behavioral decision making has a smaller effect, the PoA \emph{increases} as the budget increases. % (e.g. at very high budget, the total system loss at $\alpha = 1$ is $8\times 10^{-9}$ while it is about $10^{-7}$ at $\alpha = 0.6$). 
The intuition %at higher budgets 
is that given very high budgets, the denominator (i.e., social optimum) goes to zero much faster than the numerator (i.e., total loss at PNE of behavioral players).
%PN(10/23/18): this is interesting; can you add an intuitive explanation of why POA is higher at higher budgets?
%Mus(10/24/18): Done
%PN(10/28/18): good point, thanks. 
This analysis quantifies when central planning is likely to yield the greatest benefit in securing an interdependent system---when the defenders are highly behavioral and have high individual security budgets. 
%PN(10/23/18): I have the same comment as A.6 for this experiment too. In fact experiment B.1 is pretty much making the same point that higher interdependency makes things worse. Is there a reason why this is adding to that insight? Is something less expected emerging when we increase the number of interdependent edges?
%Mus(10/24/18): Good point. I see your point but I think actually experiment B.1 has a mix of increasing target asset and interdependency and comparing two different attack graphs but here that it only interdependency parameter control. 
%PN(10/28/18): I see, got it. 



\begin{figure*}[t]
\begin{minipage}[t]{1.0\textwidth}
\begin{minipage}[t]{0.32\textwidth}
 \includegraphics[width=\linewidth]{Figures/P_O_A_alpha.pdf}
  \caption{A comparison of optimistic Price of Anarchy for different available security budgets. We observe that Price of Anarchy increases as the player becomes more behavioral especially for higher budget. Here, central planner is non-behavioral.}
 \label{fig:POA_Behavioral_Scada}
 \end{minipage}%
    \hfill%
\begin{minipage}[t]{.32\textwidth}
\centering
\includegraphics[width=\linewidth]{Figures/Social_Individual_Budgets.pdf}
  \caption{A comparison of expected losses between centralized and distributed decision making. Social planning is most effective under moderate total budget and high budget asymmetry between defenders, and with behavioral defenders.}
  \label{fig:Central_Behavioral_Scada}
\end{minipage}\hfill    
\begin{minipage}[t]{0.32\textwidth}
     \includegraphics[width=\linewidth]{Figures/Sensitivity_Scada.pdf}
  \caption{ The percentage of investments on non-critical (NC) edges vs the sensitivity ratio (SR) between non-critical to critical edges, for different $\alpha$ in the SCADA attack graph.}
 \label{fig:sensitivity-exp-Scada}
  \end{minipage}
  \end{minipage}
\end{figure*}


